AIforCOVID: predicting the clinical outcomes in patients with COVID-19 applying AI to chest-X-rays. An Italian multicentre study

Recent epidemiological data report that worldwide more than 53 million people have been infected by SARS-CoV-2, resulting in 1.3 million deaths. The disease has been spreading very rapidly and few months after the identification of the first infected, shortage of hospital resources quickly became a problem. In this work we investigate whether chest X-ray (CXR) can be used as a possible tool for the early identification of patients at risk of severe outcome, like intensive care or death. CXR is a radiological technique that compared to computed tomography (CT) it is simpler, faster, more widespread and it induces lower radiation dose. We present a dataset including data collected from 820 patients by six Italian hospitals in spring 2020 during the first COVID-19 emergency. The dataset includes CXR images, several clinical attributes and clinical outcomes. We investigate the potential of artificial intelligence to predict the prognosis of such patients, distinguishing between severe and mild cases, thus offering a baseline reference for other researchers and practitioners. To this goal, we present three approaches that use features extracted from CXR images, either handcrafted or automatically by convolutional neuronal networks, which are then integrated with the clinical data. Exhaustive evaluation shows promising performance both in 10-fold and leave-one-centre-out cross-validation, implying that clinical data and images have the potential to provide useful information for the management of patients and hospital resources.

==> AIforCOVID_ arxiv/altretabelle.tex <==

\begin{table}[]
\caption{Overview of acquisition metadata}
\label{tab:acquisitionmetadata}
\begin{tabular}{|l|l|}
\hline
 & \textbf{Number of Patients} \\ \hline
 \textbf{Pixel Spacing} & \\ \hline
{[}0.1, 0.1{]} & 92 \\ \hline
{[}0.10, 0.10{]} & 114 \\ \hline
{[}0.136500000954, 0.136500000954{]} & 1 \\ \hline
{[}0.139, 0.139{]} & 6 \\ \hline
{[}0.144, 0.144{]} & 1 \\ \hline
{[}0.1461981383905, 0.1461981383905{]} & 1 \\ \hline
{[}0.1489667458432, 0.1489667458432{]} & 1 \\ \hline
{[}0.14948, 0.14948{]} & 1 \\ \hline
{[}0.15, 0.15{]} & 364 \\ \hline
{[}0.15000000596, 0.15000000596{]} & 7 \\ \hline
{[}0.159999996424, 0.159999996424{]} & 113 \\ \hline
{[}0.168, 0.168{]} & 20 \\ \hline
{[}0.20, 0.20{]} & 1 \\ \hline
{[}0.20000000298, 0.20000000298{]} & 21 \\ \hline
nan & 87 \\ \hline
\textbf{Bits Allocated} & \textbf{} \\ \hline
16 & 830 \\ \hline
\textbf{Bits Stored} & \textbf{} \\ \hline
10 & 112 \\ \hline
12 & 294 \\ \hline
14 & 387 \\ \hline
16 & 37 \\ \hline
\textbf{View Position} & \textbf{} \\ \hline
AP & 187 \\ \hline
nan & 386 \\ \hline
PA & 90 \\ \hline
(blank) & 167 \\ \hline
\textbf{Modality} & \textbf{} \\ \hline
CR & 414 \\ \hline
DX & 407 \\ \hline
OT & 9 \\ \hline
\end{tabular}
\end{table}

==> AIforCOVID_ arxiv/clinicaltable.tex <==


 

\begin{table}[]
\caption{Description of the clinical data available within the repository.
First and second columns report variables label and description. Summary statistics for the overall population and for the two patients groups are reported in the following columns. 
For continuous variables median and interquartile range are reported, for categorical variables proportions are reported. Feature names followed by '+' were not used for the analysis described in this work.P-values lower than 0.05 were considered significant. * Mann-Whitney U test. $\dagger$ z-test for proportions with Yates continuity correction. $\ddagger$ Fisher exact test.  }
\label{tab:databaseinformation}
\begin{adjustbox}{angle=90} 
\resizebox{1.5\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l}
\toprule
\multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\textbf{Description}} & %\multirow{2}{*}{
\textbf{Overall-}%}
& \multirow{2}{*}{\textbf{Mild-group          (A)}} & \multirow{2}{*}{\textbf{Severe-group     (B)}} & \textbf{A vs B} & %\multirow{2}{*}{
\textbf{Missing }%} 
\\ 
 &  & \textbf{population} &  &  & \textbf{p-value} & \textbf{data (\%)} \\ 
\midrule
\textbf{Active   cancer in the last 5 years} & Patient had active cancer in the last 5 years (\% reported) & 7\% & 5\% & 8\% & \textless{}0.05\dagger & 1.4 \\ \hline
\textbf{Age} & Patient's age (years) & 64; 54-77 & 60; 49-72 & 70; 60-79 & \textless{}0.001* & 0 \\\hline
\textbf{Atrial Fibrillation} & Patient had atrial fibrillaton (\% reported) & 9\% & 5\% & 11\% & \textless{}0.01\dagger & 2.2 \\ \hline
\textbf{Body temperature ($^{\circ}$C)} & Patients temperature at admission (in $^{\circ}$C) & 38; 37-38 & 38; 37-38 & 38; 37-38 & 0.171 & 8.8 \\ \hline
\textbf{Cardiovascular Disease} & Patient had cardiovascular diseases (\% reported) & 35\% & 23\% & 40\% & \textless{}0.001\dagger & 1.7 \\ \hline
\textbf{Chronic Kidney disease} & Patient had chronic kidney disease (\% reported) & 6\% & 4\% & 9\% & \textless{}0.01\dagger & 1.4 \\ \hline
\textbf{COPD} & Chronic obstructive pulmonary disease (\% reported) & 7\% & 4\% & 10\% & \textless{}0.01\dagger & 1.4 \\ \hline
\textbf{Cough} & Cought (\%yes) & 54\% & 59\% & 50\% & \textless{}0.05\dagger & 0.5 \\ \hline
\textbf{CRP} & C-reactive protein concentration (mg/dL) & 57; 24-119 & 42; 17-75 & 103; 48-163 & \textless{}0.001* & 3.5 \\ \hline
\textbf{Days Fever} & Days of fever up to admission (days) & 3; 2-4 & 3; 2-4 & 3; 2-3 & 0.289 & 10.96 \\  \hline
\textbf{D-dimer} & D-dimer amount in blood & 632; 352-1287 & 549; 262-909 & 820; 438-2056 & \textless{}0.001* & 77.6 \\ \hline
\textbf{Death+} & Death of patient occurred during hospitalization for any cause & 168 & 0 & 168 & - & - \\ \hline
\textbf{Dementia} & Patient had dementia (\% reported) & 4\% & 3\% & 6\% & 0.087 & 1.8 \\ \hline
\textbf{Diabetes} & Patient had diabetes (\% reported) & 16\% & 10\% & 21\% & \textless{}0.001\dagger & 1.4 \\ \hline
\textbf{Dyspnea} & Patient had intense tightening in the chest, air hunger, difficulty & 50\% & 37\% & 62\% & \textless{}0.001\dagger & 0.4 \\
&  breathing, breathlessness or a feeling of suffocation (\%yes)& & & & & \\ \hline
\textbf{Fibrinogen} & Fibrinogen concentration in blood (mg/dL) & 607; 513-700 & 550; 473-658 & 615; 549-700 & \textless{}0.001* & 73.6 \\ \hline
\textbf{Glucose} & Glucose concentration in blood (mg/dL) & 110; 96-130 & 104; 93-121 & 114; 101-139 & \textless{}0.001* & 20.6 \\ \hline
\textbf{Heart Failure} & Patient had heart failure (\% reported) & 2\% & 1\% & 3\% & 0.157 & 2.3 \\ \hline
%\textbf{Hospital} & Hospital identification code & - & - & - & - &  \\ \hline
\textbf{Hypertension} & Patient had high blood pressure (\% reported) & 46\% & 38\% & 54\% & \textless{}0.001\dagger & 1.4 \\ \hline
%\textbf{Image File} & name of image file & - & - & - & - &  \\ \hline
\textbf{INR} & International Normalized Ratio & 1.13; 1.07-1.25 & 1.11; 1.06-1.20 & 1.15; 1.08-1.28 & 0.004* & 28.8 \\\hline 
\textbf{Ischemic Heart Disease} & Patient had ischemic heart disease (\% reported) & 15\% & 11\% & 18\% & \textless{}0.01\dagger & 18.3 \\ \hline
\textbf{LDH} & Lactate dehydrogenase concentration in blood (U/L) & 320; 249-431 & 271; 214-323 & 405; 310-527 & \textless{}0.001* & 24.6 \\ \hline
$\mathbf{O_2}$ \textbf{(\%)} & Oxygen percentage in blood (\%) & 95; 90-97 & 96; 94-98 & 92; 87-96 & \textless{}0.001* & 16.5 \\ \hline
\textbf{Obesity} & Patient had obesity (\% reported) & 9\% & 6\% & 11\% & 0.058 & 36.1 \\ \hline
$\mathbf{PaCO_2}$ & Partial pressure of carbon dioxide in arterial blood (mmHg) & 33; 30-36 & 34; 30-37 & 33; 30-35 & 0.116 & 15.4 \\ \hline
$\mathbf{PaO_2}$ & Partial pressure of oxygen in arterial blood (mmHg) & 69; 59-80 & 73; 67-81 & 64; 54-76 & \textless{}0.001* & 15.3 \\ \hline
\textbf{PCT} & Platelet count (ng/mL) & 0.19; 0.09-0.56 & 0.09; 0.05-0.26 & 0.28; 0.13-0.72 & \textless{}0.001* & 71.8 \\ \hline
\textbf{pH} & Blood pH & 7; 7-7 & 7; 7-7 & 7; 7-7 & \textless{}0.001* & 17.3 \\ \hline
\textbf{Position+} & Patient position during chest x-ray (\%supine) & 78\% & 68\% & 87\% & \textless{}0.001\dagger & 0 \\\hline
\textbf{Positivity at admission} & Positivity to the SARS-CoV-2 swab at the admission time  & 95\% & 94\% & 96\% & 0.142 & 4.7 \\ 
& (\%   positive)& & & & &\\ \hline
\textbf{Prognosis} & Patient outcome, see section \ref{sec:materials}  (\% cases)& - & 46.8\% & 53.2\% & 0.468\dagger & 0.0 \\
\hline
\textbf{RBC} & Red blood cells count (10\textasciicircum{}9/L) & 4.65; 4.26-5.07 & 4.70; 4.34-5.11 & 4.59; 4.13-5.03 & \textless{}0.001* & 3.0 \\ \hline
\textbf{Respiratory Failure} & Patient had respiratory failure (\% reported) & 1\% & 100\% & 2\% & 0.131 & 19.0 \\ \hline
%\textbf{Row Number} & Incremental row number in the data table & - & - & - & - &  \\\hline
% Non necessario inserire il Row Number tra le variabili
$\mathbf{SaO_2}$ & arterial oxygen saturation (\%) & 95; 91-97 & 96; 94-98 & 92;87-96 & \textless{}0.001* & 59.2 \\ \hline
\textbf{Sex} & Patient's sex (\%males) & 68\% & 59\% & 75\% & \textless{}0.001\dagger & 0 \\ \hline
\textbf{Stroke} & Patient had stroke (\% reported) & 4\% & 3\% & 4\% & 0.447 & 2.3 \\ \hline
\textbf{Therapy Anakinra+} & Patient was treated with Anakinra (\%yes) & 100\% & 0\% & 0\% & - & 10.8 \\ \hline
\textbf{Therapy anti-inflammatory+} & Patient was treated with anti-inflammatory drugs & 55\% & 53\% & 57\% & 0.243 & 13.5 \\
&therapy   (\%yes) & & & & & \\ \hline
\textbf{Therapy antiviral+} & Patient was treated with antiviral drugs (\%yes) & 47\% & 44\% & 50\% & 0.129 & 10.7 \\ \hline
%\textbf{Therapy\_Eparine} & patient was treated with eparine   (no; yes; prophylactic treatment;  & 408; 83; 202; 28 & 264; 30; 62; 4 & 144; 53; 140; 24 & - & 13.4 \\ & therapeutic treatment) & & & & & \\ \hline
 
\textbf{Therapy Eparine+} & Patient was treated with eparine   (no; yes; prophylactic  & 56.6\%;	11.5\%;	 &	73.3\%;	8.3\%; &	39.9\%;	14.7\%;	
 & \textless{}0.001\ddagger & 13.4 \\ 
 & treatment; therapeutic treatment) &28\%;	3.9\% & 	17.2\%;	1.1\%&38.8\%;	6.6\% & & \\ \hline
 
\textbf{Therapy hydroxychloroquine+} & Patient was treated with hydroxychloroquine (\%yes) & 59\% & 56\% & 62\% & 0.118 & 11.6 \\\hline
\textbf{Therapy Tocilizumab+} & Patient was treated with Tocilizumab (\%yes) & 9\% & 2\% & 15\% & \textless{}0.001\dagger & 12.4 \\ \hline
\textbf{WBC} & White blood cells count (10\textasciicircum{}9/L) & 6.30; 4.73-8.42 & 5.58; 4.32-7.17 & 7.10; 5.25-9.80 & 0.012* & 0.7\\
\bottomrule
\end{tabular}}
%\captionof{table}{Table caption}% Add 'table' caption
\end{adjustbox}
\end{table}



\begin{comment}
\begin{table}[]
\caption{Population demographic characteristics.  *patients of sever-group were significantly (p\textless{}0.01) older than mild-group. \# in all groups females were always significantly (p\textless{}0.01) older than males}
\label{tab:populationdemographic}
\centering
\begin{tabular}{c|c|c|c|c}
\hline
\toprule
 & \multirow{2}{*}{\textbf{Number of patients (female)}} & \multicolumn{3}{c}{\textbf{Age}} \\\cline{3-5}
 &  & \textbf{Overall} & \textbf{Female \#} & \textbf{Male} \\
 \midrule
\textbf{Mild} & 383 (157) & 60 (49-72) years* & 63 (50-76) years & 59 (48-69) years \\ \hline
\textbf{Severe} & 440 (109) & 70 (60-79) years* & 78 (67-85) years & 67 (57-76) years \\ \hline
\textbf{Death} & 169 (47) & 78 (68-84) years & 82 (78-88) years & 76 (66-82) years \\ 
\bottomrule
\textbf{Overall} & 823 (266) & 64 (54-77) years & 70 (57-80) years & 64 (53–74) years \\ 
\bottomrule
\end{tabular}
\end{table}

\end{comment}





==> AIforCOVID_ arxiv/images/figureGradCAM.tex <==
\begin{figure}
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=.8\linewidth]{images/LieveGradCam_tutti_neuroni}
                \caption{Mild class, all neurons}
                \label{fig:MildClassALLNeurons}
        \end{subfigure}%
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=.8\linewidth]{images/LieveGradCam_soloAttivati_neuroni}
                \caption{Mild class, 40 most selected neurons}
                \label{fig:MildClass40Neurons}
        \end{subfigure}%
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=.8\linewidth]{images/SevereGradCam_tutti_neuroni}
                \caption{Severe class, all neurons}
                \label{fig:SevereClassALLNeurons}
        \end{subfigure}%
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=.8\linewidth]{images/SevereGradCam_soloAttivati_neuroni}
                \caption{Severe class, 40 most selected neurons}
                \label{fig:SevereClass40Neurons}
        \end{subfigure}
        \caption{Two examples of the activation maps provided by the Grad-CAM approach, using all the neurons in the dense layer of the CNN dense layer or all the 40  neurons selected by the RFECV wrapper. }
        \label{fig:GradCamHybrid}
\end{figure}


==> AIforCOVID_ arxiv/tabelleBestResults.tex <==
 
 


% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[th]
\centering
\caption{Best recognition performance attained by each of the learning methods when the experiments were executed according to the 10-fold cross-validation (20 repetitions). 
In the second column, ML and DL stands for Machine-Learning and Deep Learning, respectively. 
The last column reports the learners providing the results shown here. }
\resizebox{.99\textwidth}{!}{%
\begin{tabular}{@{}llcccl@{}}
\toprule
\textbf{Input data} & \textbf{Approach} & \textbf{Accuracy} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Learner} \\ \midrule
\multirow{2}{*}{Clinical data}  & ML        & $.757 \pm .008$ & $.760 \pm .007 $ & $.754 \pm .011 $ & SVM \\
& DL & $.684\pm	.019$&$	.753\pm	.020$&	$.654\pm .012$ & MLP \\
\midrule
\multirow{3}{*}{CXR images}     & Handcrafted &  $.658 \pm .015$&$	.676\pm.016$ & $.638\pm.019$ &  LGR\\
& Hybrid & $.728\pm.038$&$	.769\pm	.072$&$	.680\pm	.076$  & VGG-11 + RF   \\
& End-to-end  & $.742\pm.010$&$	.748 \pm.019$&$	.738\pm	.013$   &    Resnet50 \\
\midrule
\multirow{3}{*}{\begin{minipage}{1in}Clinical data  and CXR images\end{minipage}} & Handcrafted & $.755\pm	.007$&$	.758\pm	.008$&$	.753\pm	.013$ &   SVM  \\
& Hybrid & $.769\pm	.054$&$	.788\pm	.064$&$	.747\pm	.059$    &  GoogleNet +  SVM   \\
& End-to-end  & $.748\pm	.008$&$	.745\pm	.017$&$.751\pm	.015$ &   Resnet50 + MLP  \\
\bottomrule
\end{tabular}}
\label{tab:ResultsBest10CV}
\end{table}


\begin{table}[th]
\centering
\caption{Best recognition performance attained by each of the learning methods when the experiments were executed according to the LOCO cross-validation. 
In the second column, ML and DL stands for Machine-Learning and Deep Learning, respectively. 
The last column reports the learners providing the results shown here. }
\resizebox{.99\textwidth}{!}{%
\begin{tabular}{@{}llcccl@{}}
\toprule
\textbf{Input data} & \textbf{Approach} & \textbf{Accuracy} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Learner} \\ \midrule
\multirow{2}{*}{Clinical data}  & ML & $.734\pm	.044$&$	.699\pm	.158 $&$	.795\pm	.136$ & SVM \\
& DL & $.663\pm.016$&$	.709\pm	.032$&$	.644\pm	.018$ & MLP \\
\midrule
\multirow{3}{*}{CXR images}     & Handcrafted &  $.625\pm	.083$&$	.641\pm	.159$&$	.644\pm	.200$ & SVM\\
& Hybrid & $.693\pm.053$&$	.806\pm	.161	$&$.549\pm.213$  &   Vgg11 + SVM  \\
& End-to-end  & $.705\pm.010$&$	.720\pm	.011$&$	.696	\pm .015$  &  Resnet50   \\
\midrule
\multirow{3}{*}{\begin{minipage}{1in}Clinical data  and CXR images\end{minipage}} & Handcrafted & $.752\pm	.067$&$	.711\pm	.165$&$	.824\pm	.154$ &  LGR   \\
& Hybrid & $.743\pm	.061$&$	.769\pm	.189$&$	.685\pm	.155$    &  GoogleNet +  LGR   \\
& End-to-end  & $.709\pm.005$&$	.734\pm	.018$&$	.696	\pm.009$ &   Resnet50 + MLP  \\
\bottomrule
\end{tabular}}
\label{tab:ResultsBestCenter}
\end{table}

==> altretabelle.tex <==

\begin{table}[]
\caption{Overview of acquisition metadata}
\label{tab:acquisitionmetadata}
\begin{tabular}{|l|l|}
\hline
 & \textbf{Number of Patients} \\ \hline
 \textbf{Pixel Spacing} & \\ \hline
{[}0.1, 0.1{]} & 92 \\ \hline
{[}0.10, 0.10{]} & 114 \\ \hline
{[}0.136500000954, 0.136500000954{]} & 1 \\ \hline
{[}0.139, 0.139{]} & 6 \\ \hline
{[}0.144, 0.144{]} & 1 \\ \hline
{[}0.1461981383905, 0.1461981383905{]} & 1 \\ \hline
{[}0.1489667458432, 0.1489667458432{]} & 1 \\ \hline
{[}0.14948, 0.14948{]} & 1 \\ \hline
{[}0.15, 0.15{]} & 364 \\ \hline
{[}0.15000000596, 0.15000000596{]} & 7 \\ \hline
{[}0.159999996424, 0.159999996424{]} & 113 \\ \hline
{[}0.168, 0.168{]} & 20 \\ \hline
{[}0.20, 0.20{]} & 1 \\ \hline
{[}0.20000000298, 0.20000000298{]} & 21 \\ \hline
nan & 87 \\ \hline
\textbf{Bits Allocated} & \textbf{} \\ \hline
16 & 830 \\ \hline
\textbf{Bits Stored} & \textbf{} \\ \hline
10 & 112 \\ \hline
12 & 294 \\ \hline
14 & 387 \\ \hline
16 & 37 \\ \hline
\textbf{View Position} & \textbf{} \\ \hline
AP & 187 \\ \hline
nan & 386 \\ \hline
PA & 90 \\ \hline
(blank) & 167 \\ \hline
\textbf{Modality} & \textbf{} \\ \hline
CR & 414 \\ \hline
DX & 407 \\ \hline
OT & 9 \\ \hline
\end{tabular}
\end{table}

==> clinicaltable.tex <==


 

\begin{table}[]
\caption{Description of the clinical data available within the repository.
First and second columns report variables label and description. Summary statistics for the overall population and for the two patients groups are reported in the following columns. 
For continuous variables median and interquartile range are reported, for categorical variables proportions are reported. Feature names followed by '+' were not used for the analysis described in this work.P-values lower than 0.05 were considered significant. * Mann-Whitney U test. $\dagger$ z-test for proportions with Yates continuity correction. $\ddagger$ Fisher exact test.  }
\label{tab:databaseinformation}
\begin{adjustbox}{angle=90} 
\resizebox{1.5\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l}
\toprule
\multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\textbf{Description}} & %\multirow{2}{*}{
\textbf{Overall-}%}
& \multirow{2}{*}{\textbf{Mild-group          (A)}} & \multirow{2}{*}{\textbf{Severe-group     (B)}} & \textbf{A vs B} & %\multirow{2}{*}{
\textbf{Missing }%} 
\\ 
 &  & \textbf{population} &  &  & \textbf{p-value} & \textbf{data (\%)} \\ 
\midrule
\textbf{Active   cancer in the last 5 years} & Patient had active cancer in the last 5 years (\% reported) & 7\% & 5\% & 8\% & \textless{}0.05\dagger & 1.4 \\ \hline
\textbf{Age} & Patient's age (years) & 64; 54-77 & 60; 49-72 & 70; 60-79 & \textless{}0.001* & 0 \\\hline
\textbf{Atrial Fibrillation} & Patient had atrial fibrillaton (\% reported) & 9\% & 5\% & 11\% & \textless{}0.01\dagger & 2.2 \\ \hline
\textbf{Body temperature ($^{\circ}$C)} & Patients temperature at admission (in $^{\circ}$C) & 38; 37-38 & 38; 37-38 & 38; 37-38 & 0.171 & 8.8 \\ \hline
\textbf{Cardiovascular Disease} & Patient had cardiovascular diseases (\% reported) & 35\% & 23\% & 40\% & \textless{}0.001\dagger & 1.7 \\ \hline
\textbf{Chronic Kidney disease} & Patient had chronic kidney disease (\% reported) & 6\% & 4\% & 9\% & \textless{}0.01\dagger & 1.4 \\ \hline
\textbf{COPD} & Chronic obstructive pulmonary disease (\% reported) & 7\% & 4\% & 10\% & \textless{}0.01\dagger & 1.4 \\ \hline
\textbf{Cough} & Cought (\%yes) & 54\% & 59\% & 50\% & \textless{}0.05\dagger & 0.5 \\ \hline
\textbf{CRP} & C-reactive protein concentration (mg/dL) & 57; 24-119 & 42; 17-75 & 103; 48-163 & \textless{}0.001* & 3.5 \\ \hline
\textbf{Days Fever} & Days of fever up to admission (days) & 3; 2-4 & 3; 2-4 & 3; 2-3 & 0.289 & 10.96 \\  \hline
\textbf{D-dimer} & D-dimer amount in blood & 632; 352-1287 & 549; 262-909 & 820; 438-2056 & \textless{}0.001* & 77.6 \\ \hline
\textbf{Death+} & Death of patient occurred during hospitalization for any cause & 168 & 0 & 168 & - & - \\ \hline
\textbf{Dementia} & Patient had dementia (\% reported) & 4\% & 3\% & 6\% & 0.087 & 1.8 \\ \hline
\textbf{Diabetes} & Patient had diabetes (\% reported) & 16\% & 10\% & 21\% & \textless{}0.001\dagger & 1.4 \\ \hline
\textbf{Dyspnea} & Patient had intense tightening in the chest, air hunger, difficulty & 50\% & 37\% & 62\% & \textless{}0.001\dagger & 0.4 \\
&  breathing, breathlessness or a feeling of suffocation (\%yes)& & & & & \\ \hline
\textbf{Fibrinogen} & Fibrinogen concentration in blood (mg/dL) & 607; 513-700 & 550; 473-658 & 615; 549-700 & \textless{}0.001* & 73.6 \\ \hline
\textbf{Glucose} & Glucose concentration in blood (mg/dL) & 110; 96-130 & 104; 93-121 & 114; 101-139 & \textless{}0.001* & 20.6 \\ \hline
\textbf{Heart Failure} & Patient had heart failure (\% reported) & 2\% & 1\% & 3\% & 0.157 & 2.3 \\ \hline
%\textbf{Hospital} & Hospital identification code & - & - & - & - &  \\ \hline
\textbf{Hypertension} & Patient had high blood pressure (\% reported) & 46\% & 38\% & 54\% & \textless{}0.001\dagger & 1.4 \\ \hline
%\textbf{Image File} & name of image file & - & - & - & - &  \\ \hline
\textbf{INR} & International Normalized Ratio & 1.13; 1.07-1.25 & 1.11; 1.06-1.20 & 1.15; 1.08-1.28 & 0.004* & 28.8 \\\hline 
\textbf{Ischemic Heart Disease} & Patient had ischemic heart disease (\% reported) & 15\% & 11\% & 18\% & \textless{}0.01\dagger & 18.3 \\ \hline
\textbf{LDH} & Lactate dehydrogenase concentration in blood (U/L) & 320; 249-431 & 271; 214-323 & 405; 310-527 & \textless{}0.001* & 24.6 \\ \hline
$\mathbf{O_2}$ \textbf{(\%)} & Oxygen percentage in blood (\%) & 95; 90-97 & 96; 94-98 & 92; 87-96 & \textless{}0.001* & 16.5 \\ \hline
\textbf{Obesity} & Patient had obesity (\% reported) & 9\% & 6\% & 11\% & 0.058 & 36.1 \\ \hline
$\mathbf{PaCO_2}$ & Partial pressure of carbon dioxide in arterial blood (mmHg) & 33; 30-36 & 34; 30-37 & 33; 30-35 & 0.116 & 15.4 \\ \hline
$\mathbf{PaO_2}$ & Partial pressure of oxygen in arterial blood (mmHg) & 69; 59-80 & 73; 67-81 & 64; 54-76 & \textless{}0.001* & 15.3 \\ \hline
\textbf{PCT} & Platelet count (ng/mL) & 0.19; 0.09-0.56 & 0.09; 0.05-0.26 & 0.28; 0.13-0.72 & \textless{}0.001* & 71.8 \\ \hline
\textbf{pH} & Blood pH & 7; 7-7 & 7; 7-7 & 7; 7-7 & \textless{}0.001* & 17.3 \\ \hline
\textbf{Position+} & Patient position during chest x-ray (\%supine) & 78\% & 68\% & 87\% & \textless{}0.001\dagger & 0 \\\hline
\textbf{Positivity at admission} & Positivity to the SARS-CoV-2 swab at the admission time  & 95\% & 94\% & 96\% & 0.142 & 4.7 \\ 
& (\%   positive)& & & & &\\ \hline
\textbf{Prognosis} & Patient outcome, see section \ref{sec:materials}  (\% cases)& - & 46.8\% & 53.2\% & 0.468\dagger & 0.0 \\
\hline
\textbf{RBC} & Red blood cells count (10\textasciicircum{}9/L) & 4.65; 4.26-5.07 & 4.70; 4.34-5.11 & 4.59; 4.13-5.03 & \textless{}0.001* & 3.0 \\ \hline
\textbf{Respiratory Failure} & Patient had respiratory failure (\% reported) & 1\% & 100\% & 2\% & 0.131 & 19.0 \\ \hline
%\textbf{Row Number} & Incremental row number in the data table & - & - & - & - &  \\\hline
% Non necessario inserire il Row Number tra le variabili
$\mathbf{SaO_2}$ & arterial oxygen saturation (\%) & 95; 91-97 & 96; 94-98 & 92;87-96 & \textless{}0.001* & 59.2 \\ \hline
\textbf{Sex} & Patient's sex (\%males) & 68\% & 59\% & 75\% & \textless{}0.001\dagger & 0 \\ \hline
\textbf{Stroke} & Patient had stroke (\% reported) & 4\% & 3\% & 4\% & 0.447 & 2.3 \\ \hline
\textbf{Therapy Anakinra+} & Patient was treated with Anakinra (\%yes) & 100\% & 0\% & 0\% & - & 10.8 \\ \hline
\textbf{Therapy anti-inflammatory+} & Patient was treated with anti-inflammatory drugs & 55\% & 53\% & 57\% & 0.243 & 13.5 \\
&therapy   (\%yes) & & & & & \\ \hline
\textbf{Therapy antiviral+} & Patient was treated with antiviral drugs (\%yes) & 47\% & 44\% & 50\% & 0.129 & 10.7 \\ \hline
%\textbf{Therapy\_Eparine} & patient was treated with eparine   (no; yes; prophylactic treatment;  & 408; 83; 202; 28 & 264; 30; 62; 4 & 144; 53; 140; 24 & - & 13.4 \\ & therapeutic treatment) & & & & & \\ \hline
 
\textbf{Therapy Eparine+} & Patient was treated with eparine   (no; yes; prophylactic  & 56.6\%;	11.5\%;	 &	73.3\%;	8.3\%; &	39.9\%;	14.7\%;	
 & \textless{}0.001\ddagger & 13.4 \\ 
 & treatment; therapeutic treatment) &28\%;	3.9\% & 	17.2\%;	1.1\%&38.8\%;	6.6\% & & \\ \hline
 
\textbf{Therapy hydroxychloroquine+} & Patient was treated with hydroxychloroquine (\%yes) & 59\% & 56\% & 62\% & 0.118 & 11.6 \\\hline
\textbf{Therapy Tocilizumab+} & Patient was treated with Tocilizumab (\%yes) & 9\% & 2\% & 15\% & \textless{}0.001\dagger & 12.4 \\ \hline
\textbf{WBC} & White blood cells count (10\textasciicircum{}9/L) & 6.30; 4.73-8.42 & 5.58; 4.32-7.17 & 7.10; 5.25-9.80 & 0.012* & 0.7\\
\bottomrule
\end{tabular}}
%\captionof{table}{Table caption}% Add 'table' caption
\end{adjustbox}
\end{table}



\begin{comment}
\begin{table}[]
\caption{Population demographic characteristics.  *patients of sever-group were significantly (p\textless{}0.01) older than mild-group. \# in all groups females were always significantly (p\textless{}0.01) older than males}
\label{tab:populationdemographic}
\centering
\begin{tabular}{c|c|c|c|c}
\hline
\toprule
 & \multirow{2}{*}{\textbf{Number of patients (female)}} & \multicolumn{3}{c}{\textbf{Age}} \\\cline{3-5}
 &  & \textbf{Overall} & \textbf{Female \#} & \textbf{Male} \\
 \midrule
\textbf{Mild} & 383 (157) & 60 (49-72) years* & 63 (50-76) years & 59 (48-69) years \\ \hline
\textbf{Severe} & 440 (109) & 70 (60-79) years* & 78 (67-85) years & 67 (57-76) years \\ \hline
\textbf{Death} & 169 (47) & 78 (68-84) years & 82 (78-88) years & 76 (66-82) years \\ 
\bottomrule
\textbf{Overall} & 823 (266) & 64 (54-77) years & 70 (57-80) years & 64 (53–74) years \\ 
\bottomrule
\end{tabular}
\end{table}

\end{comment}




